Lightweight Encryption and Anonymous Routing in NoC based SoCs

Advances in manufacturing technologies have enabled System-on-Chip (SoC) designers to integrate an increasing number of cores on a single SoC. Increasing SoC complexity coupled with tight time-to-market deadlines has led to increased utilization of Intellectual Property (IP) cores from third-party vendors. SoC supply chain is widely acknowledged as a major source of security vulnerabilities. Potentially malicious third-party IPs integrated on the same Network-on-Chip (NoC) with the trusted components can lead to security and trust concerns. While secure communication is a well-studied problem in the computer networks domain, it is not feasible to implement those solutions on resource-constrained SoCs. In this paper, we present a lightweight encryption and anonymous routing protocol for communication between IP cores in NoC based SoCs. Our method eliminates the major overhead associated with traditional encryption and anonymous routing protocols using a novel secret sharing mechanism while ensuring that the desired security goals are met. Experimental results demonstrate that existing security solutions on NoC can introduce significant (1.5X) performance degradation, whereas our approach provides the same security features with minor (4%) impact on performance.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/comments.tex <==
\newpage

\section*{RESPONSES TO REVIEWER COMMENTS}

We would like to thank the reviewers for thorough and insightful comments. We have modified the manuscript to address various issues raised by the reviewers. This section outlines all the reviewer comments and our responses in terms of how we have addressed the issues in the modified manuscript. The modifications are marked in blue in the manuscript.

\newpage

\section*{REVIEWER COMMENTS FROM PRIOR SUBMISSION}
This paper was submitted to the Special Issue on Hardware Security of IEEE Transactions on Computers. We received a major revision for our paper TCSI-2019-12-0701.R1. Our responses for the major revision is enclosed (pages 16 - 20 of this manuscript). The revised version was acceptable by two reviewers. However, due to the concerns of the third reviewer, the paper was not recommended for publication in the special issue, and it was recommended to be submitted as a new submission to the IEEE Transactions on Computers.

We have modified the manuscript according to the reviewer comments. Our responses to the reviewer comments during both review cycles are mentioned below. Specifically, pages 14-15 provides responses to review comments when the paper was rejected, and pages 16-20 provides responses to the review comments during the major revision.

\subsection*{A. RESPONSES TO REVIEWER COMMENTS}
This section outlines the reviewer comments received when the paper was rejected (after major revision) and our responses in terms of how we have addressed those concerns in the current version of the manuscript.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer 1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 1:} I appreciate the difficulty of making substantial changes and I believe the key problems from the prior review have been clarified clear.

\vspace{3mm}

\textbf{Response:} 
Thank you for accepting our modifications and for the insightful comments to improve its quality.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer 2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 1:} The authors have addressed all my concerns in the revision.

\vspace{3mm}

\textbf{Response:} 
Thank you for finding our revised version acceptable and for the insightful comments to improve its quality.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer 3}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 1:} (regarding encryption strength), indeed the vulnerability I mentioned does not lead to the secret message being revealed. But what my comment implies is that the strength of the proposed encryption scheme is only as strong as a linear cipher. Specifically, given two secret messages M and M+x, each intermediate router will observe that payload(M+x) = payload(M) + x. This is, by definition, a linear cipher, which is weak because it can be broken via simple frequency analysis (i.e., inferring common plaintext). So if the proposed scheme is indeed only as strong as a linear cipher, then it should be compared (in terms of performance) with a baseline that uses a linear cipher, without the need for complex encryption nor handshaking nor onion routing.

\vspace{3mm}

\textbf{Response:} 
The comparison of  our encryption scheme directly with a linear cipher is not entirely accurate. The goal of the paper is to provide both data confidentiality (encryption) and route anonymity (anonymous routing). A linear cipher does not provide route anonymity. Therefore, the main comparison we do is between ``ENC-and-AR'' and ``LEARN'' (our approach), both of which provides route anonymity as well as data confidentiality. 

While we agree that when one node is considered it is a linear cipher, it is not linear from a global perspective.  This is due to the nature of the secret sharing scheme, the message is only completed at the destination when the destination adds its own portion of the secret. While in transit, every node adds its portion of the secret, providing secrecy of the message. Therefore, the attacks on linear ciphers will not work. The message will remain secret even if all the internal nodes in the route are malicious as long as the source $S$ and destination $D$ are trusted IPs. We have added this clarification in Section~\ref{ssec:security} and suggested an approach that further enhances security in Section~\ref{ssec:hide-secret}.

%Furthermore,  The “Enc-only” configuration is considered in experiments only to show that our approach is capable of providing both encryption and anonymous routing while providing performance close to existing NoC encryption (without anonymous routing) methods. \textcolor{red}{The main distinction we want to make is between ``ENC-and-AR'' and ``LEARN''.}
\vspace{3mm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
\textbf{Comment 2:} (regarding inferring source nodes), the authors respond that in mesh topologies, "from the perspective of any node, there can be more than one node that is at distance d away." This is not true if the node has awareness of from which port the packet arrives. For example, any node is immediately able to identify the source node if it receives a packet from its west input port with a distance d=1.

\vspace{3mm}

\textbf{Response:} 
We agree with the reviewer that in certain cases, one of which the reviewer has correctly pointed out, it leads to the identification of the destination node. We described it in Section~\ref{ssec:hide-onion} with a mechanism that eliminates such vulnerabilities.

\vspace{3mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
\textbf{Comment 3:} 
The new sections 6.2 and 6.3 are defenses for fundamental security vulnerabilities that should be in-place all the time. I don't think it suffices to argue that these are rare circumstances. The defenses described here in 6.2 and 6.3 should be implemented and evaluated as part of the results. Otherwise, the current performance numbers would be misleading, since the current implementation is not completely secure.

\vspace{3mm}

\textbf{Response:} 
Thank you for your comment. We agree that it would be appropriate to add these defenses and report the results. Figure~\ref{fig:discussion-improve-performance-real} shows the results that incorporates these defenses. As expected, it introduced slightly higher overhead (3\% on average across all the benchmarks) compared to the scenario where these defenses are not there. 
With enhanced security, LEARN improves NoC delay by 69\% (67\% on average) and total execution time by 34\% (27\% on average). Comparing with the results in Section~\ref{ssec:performance-evaluation}, the average total execution time improvement has been reduced by 3\% (from 30\% on average to 27\% on average) to accommodate the added security. 
%Even then, LEARN enables significant performance improvement compared to traditional approaches.
However, our results still remain consistent with the original observations in terms of drastic reduction in execution time compared to traditional approaches. We have modified Section~\ref{ssec:hide-onion} to include this discussion.

\begin{figure}[h]
\centering
\begin{subfigure}{0.85\columnwidth}
  \centering
  \includegraphics[width=1\linewidth]{images/results-legend}
\end{subfigure}\\%
\vspace{1mm}
\begin{subfigure}{1\columnwidth}
  \centering
  \includegraphics[width=1\linewidth]{images/results-improve-noc-delay}
  \caption{NoC delay}
  \label{fig:results-improve-noc-delay}
\end{subfigure}%
\hspace{1mm}
\begin{subfigure}{1\columnwidth}
  \centering
  \includegraphics[width=1\linewidth]{images/results-improve-exec-time}
  \caption{Execution time}
  \label{fig:results-improve-exec-time}
\end{subfigure}
\caption{NoC delay and execution time comparison across different security levels using real benchmarks considering the enhanced security features outlined in Section~\ref{ssec:hide-secret} and Section~\ref{ssec:hide-onion}.}
\label{fig:discussion-improve-performance-real}
\end{figure}

\vspace{3mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
\textbf{Comment 4:} (regarding bidirectional paths) was not adequately addressed, partly because my original comment was unclear. What I meant to say was that the proposed scheme only works on networks where the path from S to D is the same as the path from D to S. This is often not true; for example, in typical meshes with X-Y routing, having the same paths for S to D and D to S would result in Y-X turns that could now lead to deadlock. How is this addressed in the current implementation? How can this scheme work for general NoCs that may have these turn restrictions in place?

\vspace{3mm}

\textbf{Response:} 
Thank you for your comment. There is no possibility of a deadlock in our proposed approach. Let us consider the scenario where an architecture supports X-Y routing. In this case, the first message (RI packet) will follow X-Y routing (or any other routing scheme implemented in the NoC) during the handshaking phase. Subsequent packets (RA, RC and DATA) are routed on the same path taken by the RI packet and it is guided by the parameters distributed between intermediate nodes during different steps of the three-way handshake. Our anonymous routing protocol is intended at replacing the traditional X-Y routing protocol.

\iffalse
Modern SoCs use multiple physical NoCs to carry different types of packets [1], [2]. 
For example, the Knights Landing (KNL) architecture used in Intel Xeon-Phi processor family uses four parallel NoCs [2]. Similarly, the Tilera TILE64 architecture uses five Mesh NoCs, each used to transfer packets belonging to a certain packet type such as main memory, communication with I/O devices, and user-level scalar operand and stream communication between tiles [1].
The decision to implement separate physical NoCs is dependent on the performance versus area trade-off. If only one physical NoC is used to carry all types of packets, the packets must contain header fields such as $RI, RA, RC, DT$ to distinguish between different types. The buffer space is shared between different packet types. The SoC performance can deteriorate significantly due to these factors coupled with the increasing number of IPs in an SoC. On the other hand, contrary to intuition, due to the advancements in chip fabrication processes, additional wiring between nodes incur minimal overhead as long as the wires stay on-chip. 
Furthermore, when wiring bandwidth and on-chip buffer capacity is compared, the more expensive and scarce commodity is the on-chip buffer area. If different packet types are carried on NoC using virtual channels and buffer space is shared [3], the increased buffer spaces and logic complexity to implement virtual channels becomes comparable to another physical NoC. A comprehensive analysis of having virtual channels versus several physical NoCs is given in [4]. We have added this discussion in Section~\ref{ssec:service-noc}.


[1] Wentzlaff, D., Griffin, P., Hoffmann, H., Bao, L., Edwards, B., Ramey, C., Mattina, M., Miao, C.C., Brown III, J.F. and Agarwal, A., 2007. On-chip interconnection architecture of the tile processor. IEEE micro, 27(5), pp.15-31.

[2] Sodani, A., Gramunt, R., Corbal, J., Kim, H.S., Vinod, K., Chinthamani, S., Hutsell, S., Agarwal, R. and Liu, Y.C., 2016. Knights landing: Second-generation Intel Xeon Phi product. IEEE Micro, 36(2), pp.34-46.

[3] Diguet, J.P., Evain, S., Vaslin, R., Gogniat, G. and Juin, E., 2007, May. NOC-centric security of reconfigurable SoC. In First International Symposium on Networks-on-Chip (NOCS'07) (pp. 223-232). IEEE.

[4] Yoon, Y.J., Concer, N., Petracca, M. and Carloni, L.P., 2013. Virtual channels and multiple physical networks: Two alternatives to improve NoC performance. IEEE Transactions on computer-aided design of integrated circuits and systems, 32(12), pp. 1906-1919.

[5] Charles, S., Lyu, Y. and Mishra, P., 2019, March. Real-time detection and localization of DoS attacks in NoC based SoCs. In 2019 Design, Automation \& Test in Europe Conference \& Exhibition (DATE) (pp. 1160-1165). IEEE.
\fi
\newpage
\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection*{B. RESPONSES TO REVIEWER COMMENTS}
%We would like to thank the reviewers for thorough and insightful comments. We have modified the manuscript to address various issues raised by the reviewers. This section outlines all the reviewer comments and our responses in terms of how we have addressed the issues in the modified manuscript. The modifications are marked in blue in the manuscript.
This section outlines the reviewer comments received during the major revision for the initial submission to the Special Issue on Hardware Security of IEEE Transactions on Computers and our responses to the comments.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer 1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 1:} It is not clear why the design is lightweight in section 4. It would be better to clarify it clearly in Section 4. (i.e. How often the route discovery phase happens should be described in Section 4 rather than in the experiment part.)

\vspace{3mm}

\textbf{Response:} 
To understand why LEARN provides significant performance improvement, let us consider the overhead associated with both phases. The overhead occurs during the first (route discovery) phase that requires cryptographic operations. However, this is performed only a constant number of times (once per session). Since the route discovery phase happens only once in the beginning of a communication session, the cost for route discovery gets amortized over time. 
%The overhead during the second (data transfer) phase is primarily due to complex cryptographic operations. 
LEARN improves performance by replacing complex cryptographic operations with addition and multiplication operations that consume significantly less time during the data transfer phase. This leads to significant performance improvement.
We have modified Section~\ref{sec:learn} to include this discussion.

    
\vspace{3mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 2:} To demonstrate the effectiveness of your design, only 4 real benchmarks are too few. Adding more real applications instead of synthetic benchmarks would be better.

\vspace{3mm}

\textbf{Response:} 

We have added two more real benchmarks (OCEAN and CHOLESKY) from the SPLASH-2 benchmark suite to experimental results (Section~\ref{ssec:performance-evaluation}). The modified results are shown in Figure~\ref{fig:performance-real-2}. Figure~\ref{fig:performance-real} has been updated in the manuscript to include these two new benchmarks. 

\begin{figure}[htb]
\centering
\begin{subfigure}{0.85\columnwidth}
  \centering
  \includegraphics[width=1\linewidth]{images/results-legend}
\end{subfigure}\\%
\vspace{1mm}
\begin{subfigure}{1\columnwidth}
  \centering
  \includegraphics[width=1\linewidth]{images/results-noc-delay}
  \caption{NoC delay}
  \label{fig:results-noc-delay-2}
\end{subfigure}%
\hspace{1mm}
\begin{subfigure}{1\columnwidth}
  \centering
  \includegraphics[width=1\linewidth]{images/results-exec-time}
  \caption{Execution time}
  \label{fig:results-exec-time-2}
\end{subfigure}
\caption{NoC delay and execution time comparison across different security levels using real benchmarks.}
\vspace{-2mm}
\label{fig:performance-real-2}
\end{figure}
\color{black}
\vspace{3mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 3:} Since fewer route discovery phases are the major reason for the performance improvement, it would be better to provide more experimental results about it. For example, giving the ratios of the numbers of different packet types can show the reduction of route discovery phases compared with the existing scheme.

\vspace{3mm}

\textbf{Response:} 
When running real benchmarks, we observed a packet ratio of 1:1:1:6325 on average for $RI:RA:RC:DT$, respectively. For synthetic traffic patterns, a similar trend is observed with ratio of 1:1:1:1964. We have included these results in Section~\ref{ssec:performance-evaluation}.
    
\vspace{3mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer 2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 1:} In the proposed method, the data transfer phase follows the route discovery phase, which includes a three-way handshake process. However, the packets sent for handshake may be blocked in the NoC when the traffic is busy. How to guarantee that the possible NoC congestion will not hurt the performance?

\vspace{3mm}

\textbf{Response:} 
While the packets can get delayed due to congestion, they can never be blocked. The average packet latency when running the RADIX benchmark was 35.56 cycles. The maximum packet latency was observed to be 1792 cycles during the three-way handshake. However, the significant increase in latency was not due to congestion, but because of per-hop encryption and decryption operations required during the three-way handshake. We have already accounted for these delays when reporting performance improvement. From the response to Reviewer 1's Comment 3, we can see that the number of handshake messages (RI, RA, RC) are negligible compared to actual data packets. Therefore, the latency during the handshake gets amortized over time.

To accurately capture congestion, the NoC was modeled with 3-stage (buffer write, route compute + virtual channel allocation + switch allocation, and link traversal) pipelined routers with wormhole switching and 4 virtual channel buffers at each input port. Each link was assumed to consume one cycle to transmit packets between neighboring routers. We have included details about the experimental setup in Section~\ref{ssec:ex_setup}. 

We have added Section~\ref{ssec:service-noc} to discuss the feasibility of implementing a separate service NoC to carry out the handshake packets in parallel to data packets to further improve performance.
Modern SoCs use multiple physical NoCs to carry different types of packets [1], [2]. 
The Knights Landing (KNL) architecture used in Intel Xeon-Phi processor family uses four parallel NoCs [2]. The Tilera TILE64 architecture uses five Mesh NoCs, each used to transfer packets belonging to a certain packet type such as main memory, communication with I/O devices, and user-level scalar operand and stream communication between tiles [1].
The decision to implement separate physical NoCs is dependent on the performance versus area trade-off. If only one physical NoC is used to carry all types of packets, the packets must contain header fields such as $RI, RA, RC, DT$ to distinguish between different types. The buffer space is shared between different packet types. The SoC performance can deteriorate significantly due to these factors coupled with the increasing number of IPs in an SoC. On the other hand, contrary to intuition, due to the advancements in chip fabrication processes, additional wiring between nodes incur minimal overhead as long as the wires stay on-chip. 
Furthermore, when wiring bandwidth and on-chip buffer capacity is compared, the more expensive and scarce commodity is the on-chip buffer area. If different packet types are carried on NoC using virtual channels and buffer space is shared [3], the increased buffer spaces and logic complexity to implement virtual channels becomes comparable to another physical NoC. A comprehensive analysis of having virtual channels versus several physical NoCs is given in [4].

It is possible to use two physical NoCs - one for data ($DT$) packet transfers and the other to carry packets related to the handshake ($RI, RA, RC$). However, in our setup, the potential performance improvement from a separate service NoC was not enough to justify the area and power overhead. We envision that our security mechanism to be a part of a suite of NoC security countermeasures that can address other threat models such as denial-of-service, buffer overflow, etc. The service NoC will be effective in such a scenario where more service type packets (e.g., DoS attack detection related packets [5]) are transferred through the NoC.

[1] Wentzlaff, D., Griffin, P., Hoffmann, H., Bao, L., Edwards, B., Ramey, C., Mattina, M., Miao, C.C., Brown III, J.F. and Agarwal, A., 2007. On-chip interconnection architecture of the tile processor. IEEE micro, 27(5), pp.15-31.

[2] Sodani, A., Gramunt, R., Corbal, J., Kim, H.S., Vinod, K., Chinthamani, S., Hutsell, S., Agarwal, R. and Liu, Y.C., 2016. Knights landing: Second-generation Intel Xeon Phi product. IEEE Micro, 36(2), pp.34-46.

[3] Diguet, J.P., Evain, S., Vaslin, R., Gogniat, G. and Juin, E., 2007, May. NOC-centric security of reconfigurable SoC. In First International Symposium on Networks-on-Chip (NOCS'07) (pp. 223-232). IEEE.

[4] Yoon, Y.J., Concer, N., Petracca, M. and Carloni, L.P., 2013. Virtual channels and multiple physical networks: Two alternatives to improve NoC performance. IEEE Transactions on computer-aided design of integrated circuits and systems, 32(12), pp. 1906-1919.

[5] Charles, S., Lyu, Y. and Mishra, P., 2019, March. Real-time detection and localization of DoS attacks in NoC based SoCs. In 2019 Design, Automation \& Test in Europe Conference \& Exhibition (DATE) (pp. 1160-1165). IEEE.

\vspace{3mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 2:} In Fig. 6, the authors show the 8x8 mesh NoC used in the experiment. Is the placement of the trusted and untrusted nodes randomly generated? Will the placement of the trusted/untrusted nodes affect the efficiency of the proposed method? The evaluation part should includes the sensitivity study to this placement.

\vspace{3mm}

\textbf{Response:}
Yes, the placement of nodes is generated randomly. 
The execution time of the application depends on the amount of NoC traversals and therefore, on node placements. However, the placement of nodes affect all four scenarios (No-Security, Enc-Only, Enc-and-AR, LEARN) explored in experimental results. Therefore, we observed the same trend with different random placements.
%Since we have modelled trusted nodes randomly, it is safe to assume that they are evenly distributed.
In our experiments, the memory controllers are attached to the corner nodes simulating worst case behavior since the number of hops is maximized in that case. Address mapping is done evenly across all memory controllers so that all 8 memory controllers are accessed during simulation. If a smart address mapping is used where cores communicate with memory controllers that are close to it, better performance can be achieved [1]. However, such performance improvement equally affects all four scenarios, and therefore, LEARN will not exhibit any particular advantage/disadvantage. Furthermore, performance optimization by address/application mapping is beyond the scope of our work.

[1] Saeidi, Samira, Ahmad Khademzadeh, and Armin Mehran. "SMAP: An intelligent mapping tool for network on chip." 2007 International Symposium on Signals, Circuits and Systems. Vol. 1. IEEE, 2007.

\vspace{3mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 3:} The description for the experiment setup requires further clarification. For example, the injection rate for the real workload and synthetic traffic are not introduced.

\vspace{3mm}

\textbf{Response:} 
When running real benchmarks, the packets get injected to the NoC when there are private cache misses and the frequency of private cache misses depends on the characteristics of the benchmark. Therefore, an injection rate is not defined. However, for synthetic traffic patterns, injection rate is defined. In our experiments, we used an injection rate of 0.01 packets/node/cycle. We have included this discussion in Section~\ref{ssec:ex_setup}. We have also added details about the NoC performance model we used in our experimental setup.
    
\vspace{3mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 4:} Will the injection rate affect the efficiency of the proposed method? A sensitivity study is required.

\vspace{3mm}

\textbf{Response:} 
As discussed in the answer to Reviewer 2's Comment 3, injection rate for real benchmarks is not pre-defined, it depends on benchmark characteristics (private cache misses). We used an injection rate of 0.01 packets/node/cycle when running synthetic traffic patterns. In our method, data injection happens during the data transfer phase that comes after route discovery. Once the path is established during the route discovery phase, data packets can be sent in any rate. With an increased injection rate, performance can be affected due to congestion. However, congestion due to increase in injection rate affects all four scenarios (No-Security, Enc-Only, Enc-and-AR, LEARN shown in Figure~\ref{fig:performance-real}) and our method does not show any bias with varying injection rate when compared with No-Security configuration. To further evaluate our approach with other configurations, we have added two more real benchmarks in Section~\ref{fig:performance-real}.

\vspace{3mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer 3}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 1:} The encryption strength of data packets seems to be low, as low as a linear cipher. For each new message M, the only difference in the payload is the value of $y_0'$. And since $y_ib_i$ is fixed for all intermediate nodes and M is simply equal to their sum, then $M$ and $y_0'$ are linearly proportional. This has two implications:
1) Since the path from S to D is fixed (once established), an intermediate node (say r2) can eventually infer the secret messages based on linear proportions of observed payload values and common payload values.
2) If the proposed data encryption mechanism is indeed as weak as a linear cipher, then the evaluation should compare it against a linear cipher. Would the performance benefit of the proposed approach still be significant when compared to a simple linear cipher (since their hardware delay would likely be similar)?
The paper needs to better justify/prove that the proposed encryption is stronger, because as currently described in the paper, I'm not convinced.

\vspace{3mm}

\textbf{Response:} 
The vulnerability mentioned above does not lead to the secret message being inferred. However, this can enable a malicious intermediate node to infer a communication path. Since each intermediate node adds a constant value ($y_ib_i$) to the received $DT$ packet, the difference between incoming and outgoing $DT$ packets at each node will be the same for a given virtual circuit.
For this attack to take place, two consecutive routers have to be infected by attackers and they have to collaborate. Alternatively, a Trojan in a router has to have the ability to observe both incoming and outgoing packets at the router. While these are strong security assumptions, it is important to address this loophole.
Even in the presence of such an attack, the secret message cannot be inferred since the complete message is only constructed at the destination and according to our threat model, we assume that the source and destination IPs are trustworthy.

This can be solved by changing the shared secret at each node for each message. However, generating and distributing secrets for each node per message can incur significant performance overhead. This demands a smarter way of doing it. According to Equation~\ref{eq:lag_coef_s}, to derive a new Lagrangian coefficient $b_i$, the $x$ coordinates should be changed. The source can easily do it for each message by changing both $x_0$ and $y_0$ when a new message needs to be sent. In other words, rather than changing the point ($x_0$,$y_0$) to ($x_0$,$y_0'$), it should be changed to ($x_0'$,$y_0'$). However, the new $x_0'$ now has to be sent to each intermediate node for them to be able to calculate the new secrets using:
\begin{equation}
    b'_j = b_j \cdot \frac{x'_0}{x'_0 - x_j} \cdot \frac{x_0 - x_j}{x_0}
\end{equation}
However, we want to avoid such communications for performance as well as security concerns. An alternative is to use a function $\mathcal{F}(x_0,\delta)$ that can derive the next $x$-coordinate starting from the initial $x_0$.
\begin{equation}
    x_0' = \mathcal{F}(x_0,\delta)
\end{equation}
where $\mathcal{F}(x_0,\delta)$ can be a simple incremental function such as $\mathcal{F}(x_0,\delta) = x+\delta$. $\delta$ can be a constant. 
To increase security, $\delta$ can be picked using a psuedo-random number generator (PRNG) seeded with the same value at each iteration.
Using such a method will change the shared secrets at each iteration and that will remove correlation between incoming and outgoing packets at a node. We have added this discussion in Section~\ref{ssec:hide-secret}.

The primary goal of the paper is to provide both data confidentiality (encryption) and route anonymity (anonymous routing). A linear cipher does not provide route anonymity. The ``Enc-only" configuration is considered in experiments to show that our approach is capable of providing both encryption and anonymous routing while providing performance close to existing NoC encryption (without anonymous routing) methods.

\vspace{3mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 2:} It is unclear why the intermediate nodes need to manipulate the value of the secret message in the first place. It does not strengthen the anonymity of the source. It seems to only strengthen the anonymity of the route, but there are far simpler ways of providing anonymous routes: minimal/non-minimal non-deterministic routing algorithms have been well studied.

\vspace{3mm}

\textbf{Response:} 
The goal of changing the message at each hop is not only to provide route anonymity, but also to ensure message confidentiality.
Since data packets are not encrypted, our scheme relies on the message being different at each hop to provide message confidentiality. The message is changed at each hop by each node by adding its portion of the secret and it is only completely constructed at the destination so that any eavesdropper in the middle cannot infer the plain text of the message. The existing approaches will not be able to serve the dual objectives of route anonymity as well as message confidentiality in resource-constrained NoC-based SoCs.

%\textcolor{magenta}{directly address the question. The second part of his observation is not relevant.}
    
\vspace{3mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 3:} The proposed mechanism does not seem effective at anonymizing the source node when at the edge of the topology. Intermediate nodes can infer how far they are from the source and destination based on the size of the RA and RC packets. So even if the source/destination are never explicitly declared during the handshake, they can be easily inferred depending on the topology.

\vspace{3mm}

\textbf{Response:} 
We agree with the reviewer's comment that an intermediate node may be able to infer the distance from that node to the source/destination by looking at the RA/RC packets. However, except for the corner case where the source/destination are at the edge of a certain topology, there can be more than one choice for potential source/destination candidates. In our experiments, we use the Mesh topology in which from the perspective of any node, there can be more than one node that is at distance $d$ away. However, the attacker can reduce the set of possible source/destination candidates for a given communication stream. Therefore, this vulnerability needs to be addressed.

To address this, when the $RA$ packet is initiated at $D$, $D$ generates $m$ $\langle$nonce, key$\rangle$ pairs ($ \langle \upsilon_D^1,K_{S-D}^1 \rangle , \langle \upsilon_D^2,K_{S-D}^2 \rangle,...,\langle \upsilon_D^m,K_{S-D}^m \rangle$) and adds $m$ layers to the packet. As a result, the $RA$ packet sent from $D$ to $r2$ takes the form:
\begin{multline*}
    \{RA \concat E_{TPK_{r2}^{(i)}} ( 
    E_{OPK_S^{(i)}}(... 
    E_{OPK_S^{(i)}}( 
    E_{OPK_S^{(i)}} (\rho \concat \upsilon_D^1 \\ \concat K_{S-D}^1 ) 
    \concat \upsilon_D^2 \concat K_{S-D}^2) ...
    \concat \upsilon_D^m \concat K_{S-D}^m)
    ) \}
\end{multline*}
$D$ stores the $\langle$nonce, key$\rangle$ pairs in its key mapping table. When $S$ receives the $RA$ packet, $S$ cannot distinguish whether the $m$ pairs were generated from multiple nodes or one node. Therefore, when the $RC$ packet is generated at $S$, instead of generating $k+1$ points (corresponding to the number of nodes in the path), the number of generated points depends on the number of $\langle$nonce, key$\rangle$ pairs received. During $RC$ packet transfer, each intermediate node along the routing path stores points (VCNs and secrets) corresponding to the nonces stored in the key mapping table. As a result, nodes can receive multiple secrets which can then be used during the data transfer phase. Depending on the required level of security, $m$ can vary and also, each intermediate node can add multiple layers to the $RA$ packet. 

This method hides the correlation between the number of nodes and the length of the routing path, and therefore, eliminates the said vulnerability. However, this increases the performance penalty. Therefore, the number of extra layers should be decided after considering the security-performance trade-off. We have added this discussion in Section~\ref{ssec:hide-onion}.

\vspace{3mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 4:} The proposed scheme only works on network topologies where all links are bidirectional; since the handshaking relies on the property that the path from S to D is the same as the path from D to S. This is not often true; for example, typical meshes with X-Y routing do not satisfy this property. Is it possible for this scheme to be more general?

\vspace{3mm}

\textbf{Response:} 
Our approach is applicable in a wide variety of NoC topologies where all links are bidirectional. There are many NoC topologies with bidirectional links as evidenced by academic research [1] as well as commercial SoCs [2], [3].
%The handshaking relies on the $RI, RA,$ and $RC$ packets traversing along the same path to distribute the keys and nonces. If X-Y routing is used, the mechanism will not hold. 
We have added this clarification in Section~\ref{ssec:ex_setup} and Section~\ref{ssec:performance-evaluation}

%Once the route is established, the data packets will be routed using the virtual channel numbers. 

%Therefore, routing protocols are applicable only for handshake messages which are negligible compared to the number of data packets. When running real benchmarks, we observed a packet ratio of 1:1:1:6325 on average for $RI:RA:RC:DT$, respectively. For synthetic traffic patterns, the same trend is observed with ratio of 1:1:1:1964. 

[1] Agarwal, N., Krishna, T., Peh, L.S. and Jha, N.K., 2009, April. GARNET: A detailed on-chip network model inside a full-system simulator. In 2009 IEEE international symposium on performance analysis of systems and software (pp. 33-42). IEEE.

[2] Wentzlaff, D., Griffin, P., Hoffmann, H., Bao, L., Edwards, B., Ramey, C., Mattina, M., Miao, C.C., Brown III, J.F. and Agarwal, A., 2007. On-chip interconnection architecture of the tile processor. IEEE micro, 27(5), pp.15-31.

[3] Sodani, A., Gramunt, R., Corbal, J., Kim, H.S., Vinod, K., Chinthamani, S., Hutsell, S., Agarwal, R. and Liu, Y.C., 2016. Knights landing: Second-generation Intel Xeon Phi product. IEEE Micro, 36(2), pp.34-46.
\color{black}
\vspace{3mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 5:} No mention of the NoC configuration in the evaluation: packet types/sizes, VCs, flow control?

\vspace{3mm}

\textbf{Response:} 
We used the default gem5 and Garnet2.0 configurations for packet sizes, virtual channels and flow control. In addition to the four main types of packets described in Section~\ref{ssec:overview}, the $DT$ packets can be further divided into two categories as control and data packets. For example, in case of a cache miss, a memory request packet (control packet) is injected into the NoC and the memory response packet (data packet) consists of the data block from the memory. The address portion of a control $DT$ packet consists of 64 bits. In the data $DT$ packet, in addition to the 64-bit address, 512 bits are reserved for the data block. A credit-based, virtual channel flow control was used in the architecture. Each data VC was allocated a buffer depth of 4 whereas control VCs had a buffer depth of 1. We have included these details in Section~\ref{ssec:ex_setup}.

\vspace{3mm}

\color{black}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 6:} Missing important details of the key mapping tables. How big do the key mapping tables need to be? Do they impose a scalable overhead (should be evaluated)? What if the key mapping table for a router is full? Would the handshaking have to be blocked or discarded? If so, can this lead to deadlock/livelock scenarios?

\vspace{3mm}

\textbf{Response:} 
    The key mapping table adds a row for each session. Therefore, the size of the key mapping table is linearly proportional to the number of sessions. If at design time, it is decided to have a fixed size for the key mapping table, it is possible for the key mapping table at a router to be full after adding sessions, and in that case, new sessions cannot be added through that router. Therefore, the size has to be decided according to the communication requirements.
    
\newpage
    The maximum number of communication pairs in an $8 \times 8$ Mesh is $\binom{64}{2} \times 2 = 4032$ (assuming two-way communication between any pair out of the 64 nodes). Depending on the address mapping, only some node pairs (out of all the possible node pairs) communicate. Our simulations consisted of 256 unique node pairs. 
    %16 IPs x 8 MCs x 2 two way communication = 256
    In the worst case, if we assume each communication session has one common router, the key mapping table should be $256 \times row\_size$ big. If each entry in the key mapping table is 128 bits, the total size becomes 20kB. However, in reality, not all communication sessions overlap. It is also important to note that except for the Session ID in the key mapping table, the other entries can be overwritten once route discovery phase is complete.
    Therefore, it is possible to allocate a fixed size key mapping table during design time and yet keep the area overhead low. We have added this discussion in Section~\ref{ssec:key-mapping-overhead}.
\vspace{3mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Comment 7:} Are TPKs also implemented as trapdoors? And are they also one-time use? These should be clarified, because I imagine there may be potential complications in the handshaking protocol if TPKs were not one-time trapdoors.

\vspace{3mm}

\textbf{Response:} 
    Thank you for your comment. The TPKs are intended to be one-time trapdoors. We have added this clarification in Section~\ref{ssec:route-discovery}.

\vspace{3mm}

==> sections/related_work.tex <==
\section{Background and Related Work} \label{sec:background}

\subsection{Related Work} \label{ssec:related_work}

Related work:
\begin{itemize}
    \item ANODR: Anonymous On Demand Routing with Untraceable Routes for Mobile Adhoc Networks~\cite{kong2003anodr}
    \item AASR: Authenticated Anonymous Secure Routing for MANETs in Adversarial Environments~\cite{liu2014aasr}
    \item \textcolor{blue}{OLAR: On-demand Lightweight Anonymous Routing in MANETs~\cite{qin2008olar}}
\end{itemize}

\subsection{Symmetric and Asymmetric Key Cryptography} \label{ssec:intro_crypto}

\subsection{Secret Sharing using Polynomial Interpolation} \label{ssec:intro_ss}

The secret sharing mechanism confirms to a $(k,n)$ threshold. The $(k,n)$ threshold means that if the secret
$M$ is divided into $n$ parts, then the knowledge of any $k$ parts or more makes $M$ easily computable but knowledge of any $k-1$ parts or fewer leaves $M$ completely undetermined. The $(k,n)$ threshold can be satisfied by Lagrangian polynomials. Given a set of $k$ points $(x_0,y_0), (x_1,y_1), ..., (x_{k-1},y_{k-1})$  where $x_i \neq x_j$ $(0 \leq i, j \leq k-1)$, a unique interpolation polynomial of degree $k-1$ can be constructed as:
\begin{equation} \label{eq:lag_sum}
    L(x) = \sum_{j=0}^{k-1} l_j(x) \cdot y_j,
\end{equation}
where
\begin{equation} \label{eq:lag_coef}
    l_j(x) = \prod_{i=0, i \neq j}^{k-1} \frac{x-x_i}{x_j - x_i}
\end{equation}

In, \ref{eq:lag_sum} and \ref{eq:lag_coef}, the interpolation polynomial $L(x)$ is in Lagrangian form and $l_j(x)$ is a Lagrangian basis polynomial. The polynomial cannot be constructed unless all the $k$ points are acquired. For example, to share the secret $M$ among $k$ participants, we can select a polynomial $L(x) = a_0 + a_1x + a_2x^2 + ... + a_{k-1}x^{k-1}$ where $a_0=M$ and all other coefficients are randomly selected values, i.e., $M = L(0)$. Then we randomly select $k$ points $(x_0,y_0), (x_1,y_1), ..., (x_{k-1},y_{k-1})$ on the curve of $L(x)$ and compute the corresponding Lagrangian coefficients $l_j(0) (0 \leq j \leq k-1)$. These values are distributed to the $k$ participants, respectively, so that each of them gets a point and its Lagrangian coefficnet. only if all participants share their secrets (i.e., points), can they derive the secret $M$ by using the following formula;
\begin{equation} \label{eq:find_m}
    M = \sum_{j=0}^{k-1} l_j(0) \cdot y_j,
\end{equation}
where $l_j(0)$ can be obtained by substituting $x=0$ in \ref{eq:lag_coef}.



\subsection{Routing Protocol}

Two main parts:
\begin{itemize}
    \item Route discovery: Send an onion packet and discover route, distribute the coefficients among participants.
    \item Message transfer: Transfer messages with just additions and multiplications.
\end{itemize}

\color{red}
\begin{itemize}
    \item How to justify the route discover phase? Is it a one time thing done in the beginning? Or we do it in phases? If yes, how to decide which phase to shift?
\end{itemize}

\color{black}

==> sections/routing_bkp.tex <==
\section{Anonymous Routing and Encryption Protocol} \label{sec:trust_aware_routing}

\subsection{Overview - Routing Protocol}

Two main parts:
\begin{itemize}
    \item Route discovery: Send an onion packet and discover route, distribute the coefficients among participants.
    \item Message transfer: Transfer messages with just additions and multiplications.
\end{itemize}

\color{red}
\begin{itemize}
    \item How to justify the route discover phase? Is it a one time thing done in the beginning? Or we do it in phases? If yes, how to decide which phase to shift?
    \item if we don't use nonces, we cant have multiple paths overlapping together But to have nonces, somenoe has to make sure nonces are generated! who? what guaranteers to say that a random number that was generated will not be generated again? do we even have to address this? Can we just say that a nonce is generated and get away with it?
    \item Can we write the paper in two halves? First discuss without using a nonce for VCI and with B-OLAR. Then point out the drawbacks and propose the more advanced scheme.
\end{itemize}

\color{black}

OLAR applies a distributed \textit{polynomial interpolation}~\cite{shamir1979share} mechanism to achieve anonymous message transfer without per-hop encryptions and decryptions. The only task for a forwarder is to perform additions and multiplications, which cost much less than traditional cryptographic operations. Meanwhile, the messages traveling through a certain path have different appearances at different hops. Any forwarding router can not see the original messages as they are reconstructed only at the destination. This design makes the messages untraceable not only to outside attackers but also to malicious insiders.

Normally, a routing protocol has two phases;
\begin{itemize}
    \item route discovery phase
    \item message transfer phase
\end{itemize} 

During the route discovery phase, the source generates a polynomial for each path that is found by route requests flooding. Then the selected points on the curve which represents the polynomial are distributed to the forwarders on the path. With these points, the forwarders are able to forward messages to the destination without revealing the secret contained in it. The only operation they need to do is addition, instead of decryption and encryption. However, only the destination can get the original messages at the end.

Four main types of packets sent on the network during the two phases; Three packets for the three-way handshake completed during the route discovery phase and another packet to transfer data during the message transfer phase.
\begin{itemize}
    \item $RI$ (route initiate) - initialize a conversation with the destination router $D$.
    \item $RA$ (route accept) - Destination accepts incoming connection
    \item $RC$ (route confirm) - share route configuration information with intermediate routers
    \item $DT$ (data) - data packets
\end{itemize}

\subsection{Nomenclature} \label{ssec:nomenclature}

\begin{table}[H]
\begin{tabular}{|l|l|}
\hline
$OPK_S^{(i)}$ & \begin{tabular}[c]{@{}l@{}}one-time public key used by the source to \\ uniquely identify an $RA$\end{tabular} \\ \hline
$OSK_S^{(i)}$  & \begin{tabular}[c]{@{}l@{}}the corresponding secret key of $OPK_S^{(i)}$\end{tabular}                          \\ \hline
$\rho$ & a random number generated by the source                                                                     \\ \hline
$PK_D$ & the global public key of the destination                                                                    \\ \hline
$SK_D$ & \begin{tabular}[c]{@{}l@{}}the corresponding secret key of $PK_D$\end{tabular}                         \\ \hline
$TPK_A^{(i)}$  & temporary public key of node $A$                                                                \\ \hline
$TSK_A^{(i)}$  & \begin{tabular}[c]{@{}l@{}}the corresponding secret key of $TPK_A^{(i)}$ \end{tabular}                            \\ \hline
$K_{S-A}$  & a shared key with source $S$ in node $A$'s key pool                                                             \\ \hline
$\upsilon_A$ & a nonce randomly generated by node $A$                                                          \\ \hline
$b_i$ & Lagrangian coefficient of point $(x_i,y_i)$                                                                          \\ \hline
$E_K(M)$ & a message $M$ encrypted using the key $K$ \\
\hline
\end{tabular}
\end{table}

\subsection{Route discovery}

In order to initialize a conversation with the destination $D$, the source $S$ broadcast a route initiate ($RI$) packet. It has the following format;
\begin{equation*}
    \{RI \concat OPK_S^{(i)} \concat E_{PK_D} (OPK_S^{(i)} \concat \rho ) \concat TPK_S^{(i)} \}
\end{equation*}
$RI$ is the message type (route initiate). $OPK_S^{(i)}$ is a one-time public key of the source router, which is changed in every $RI$ sent by the source. Thus, each $RI$ has a unique $OPK_S^{(i)}$, which can be used as its identifier. When broadcasting an $RI$, the source stores the $OPK_S^{(i)}$ and its corresponding secret key $OSK_S^{(i)}$ in its
route request table. $\rho$ is a randomly generated number. It is wrapped together with $OPK_S^{(i)}$ by the destination's global public key $PK_D$ as a global trapdoor [6]. Only the destination can open the trapdoor and acquire $\rho$, which is necessary for the destination to get authenticated by the
source. Finally, $TPK_S^{(i)}$ is a temporary public key of the
router forwarding the $RI$. Initially, it is a temporary public key selected by $S$.

After router $r1$ receives the $RI$, it checks whether it is a duplicated packet by looking up the $OPK_S^{(i)}$ in its key mapping table. If the $RI$ has been received previously, the message is simply discarded. Otherwise, $r1$ tries to open the trapdoor using its own secret key.
If it fails, $r1$ replaces $TPK_S^{(i)}$ with a temporary public
key $TPK_{r1}^{(i)}$ and broadcasts the following message:
\begin{equation*}
    \{RI \concat OPK_S^{(i)} \concat E_{PK_D} (OPK_S^{(i)} \concat \rho ) \concat TPK_{r1}^{(i)} \}
\end{equation*}
In addition, router $r1$ also fills in its key-mapping table with $OPK_S^{(i)}$, $TPK_S^{(i)}$, and $TPK_{r1}^{(i)}$. These values will be used to set up a virtual circuit when r1 receives a reply
message from the destination.

Eventually, when $D$ receives the $RI$ and opens the trapdoor using its secret key $SK_D$, it has to compare the $OPK_S^{(i)}$ in $E_{PK_D} (OPK_S^{(i)} \concat \rho )$ with that in plain text to verify the integrity of the $RI$. If these two keys are different, $D$ ignores this $RI$; otherwise, $D$ replies a route accept ($RA$) with the following format:
\begin{equation} \label{eq:ra_init}
    \{RA \concat E_{TPK_{r2}^{(i)}} ( E_{OPK_S^{(i)}} (\rho \concat \upsilon_D \concat K_{S-D} )) \}
\end{equation}
In \ref{eq:ra_init}, $RA$ indicates the message type (a route accept). $\upsilon_D$ is a randomly generated nonce which is later used as a virtual circuit identifier (VCI). A symmetric key $K_{S-D}$ is also randomly selected to share with the source. The message is encrypted by $OPK_S^{(i)}$, so that only the source can decrypt it, and then it is encrypted by router $r2$’s public key $TPK_{r2}^{(i)}$.

To keep track of the generated nonce and corresponding keys, D stores $\upsilon_D$ and $K_{S-D}$
in its key mapping table. In addition, $D$ also creates an
entry in its routing table indexed by the VCI number
$\upsilon_D$ (shown in Figure \ref{fig:}). Once the $RA$ is received by
$r2$, it decrypts the message using its temporary secret
key $TSK_{r2}^{(i)}$. Then, $r2$ generates a random nonce $\upsilon_{r2}$,
selects a shared key $K_{S-r2}$, appends them to the onion,
and encrypts the onion with $OPK_S^{(i)}$. Finally, $r2$ looks
up the temporary public key of its predecessor ($TPK_{r1}^{(i)}$)
in the key-mapping table and encrypts the onion using
$TPK_{r1}^{(i)}$. The $RA$ sent by $r2$ has the following format:
\begin{equation} \label{eq:ra_by_r2}
    \{RA \concat E_{TPK_{r1}^{(i)}} (E_{OPK_S^{(i)}}( E_{OPK_S^{(i)}} (\rho \concat \upsilon_D \concat K_{S-D} ) \concat \upsilon_{r2} \concat K_{S-r2})) \}
\end{equation}
The above mentioned procedure will continue until the reply message reaches the source (see the packet information on each hop in Figure \ref{fig:}). When the source receives
the $RA$, it first decrypts the message using $TSK_{S}^{(i)}$
and then uses $OSK_S^{(i)}$ to strip the onion layer-by-layer.
Eventually, the source will retrieve all the shared keys
and VCI numbers as well as the number $\rho$. If the destination gets authenticated successfully by providing the correct $\rho$, the source router will then create a route confirm message ($RC$).

Before sending the $RC$ message, the source $S$ generates $k+1$ points on a polynomial of degree $k$, say $L(x)$, as shown in Figure!\ref{fig:}, where $k+1$ equals the total number of nodes on the path from $S$ to $D$. Then the source calculates the Lagrangian coefficients by $b_0, b_1, ... , b_k$ for these points using:
\begin{equation} \label{eq:lag_coef_s}
    b_j = \prod_{i=0, i \neq j}^{k} \frac{x_i}{x_i - x_j}
\end{equation}
Noted that $b_j = l_j(0)$ in~\ref{eq:lag_coef}. The source $S$ creates and sends a $RC$ packet with the following format:
\begin{multline} \label{eq:rc_msg}
    \{RC \concat \upsilon_{r1} \concat E_{K_{S-r1}}(x_1 \concat y_1 \concat b_1 \concat \upsilon_{r2} \concat E_{K_{S-r2}}(x_2 \concat y_2 \concat b_2 \concat \upsilon_{D} \\ \concat E_{K_{S-D}} (x_3 \concat y_3 \concat b_3)) ) \}
\end{multline}
$RC$ is the message type (route confirmation) and the
rest of ~\ref{fig:rc_msg} is an onion structure. In this onion, each nonce $\upsilon_i$ is followed by the information encrypted using
a pairwise shared key $K_{S-*}$, where $*$ represents $r1$, $r2$, or
$D$. The pair ($\upsilon_i, K_{S-*}$) is generated by the $i^{th}$ successor of the source along the route to the destination and the last pair $(\upsilon_{D}, K_{S-D})$ belongs to $D$. Therefore, each router receiving the $RC$ can determine if the packet is for itself by checking its key mapping table. Based on the decrypted message, each node can fill in its routing table with incoming VCI number and outgoing VCI number. For example, $r1$ can decrypt the message and build an entry in its routing table as shown in Figure ~\ref{fig:}, where $\upsilon_{r1}$
is the incoming VCI number, $\upsilon_{r2}$ is the outgoing VCI number, and the tuple $(x_1, y_1, b_1)$ is the secret used in data transfer. In this way, each node can build up its own routing table.

\subsection{Data transfer}

Based on the path set up in the route discovery phase,
messages can be transferred from the source to the destination anonymously. Suppose the source $S$ has a message $M$ destined to node $D$. For example, $M$ can be
an integer, which can be mapped to a sequence of characters based on publicly known transformation settings.
During the route discovery, $k + 1$ points $(x_i, y_i)$ (where $0 \leq i \leq k$) on the curve formed by a randomly constructed polynomial $L(x)$ have been selected by $S$. Each
node on the path is distributed one of them and its corresponding coefficient $b_i$. The point $(x_0, y_0)$ and its coefficient $b_0$ are retained by $S$ itself. However, as shown in Figure~\ref{fig:}, to send the message $M$ to the destination through this path, the source $S$ needs to construct another curve of degree $k + 1$, which is determined by the original $k$
points $(x_i, y_i)(1 \leq i \leq k)$ and a new point $(0, M)$, i.e.,
the polynomial of the new curve, say $L'(x)$, must satisfy
$L'(0) = M$ and $M$ is the secret. In addition, the source
$S$ updates its own point by making $y'_0 = L'(x_0)$, which
means the new point $(x_0, y'_0)$ is also on the new curve.
According to~\ref{eq:find_m}, we can derive:
\begin{equation} \label{eq:find_m}
    M = y'_0b_0 + \sum_{i=1}^{k} b_i \cdot y_i,
\end{equation}
where $b_0, b_i$ and $y_i, (1 \leq i \leq k)$, are unchanged and retained by each node along the path. Therefore, to
transfer the message $M$ to the destination anonymously,
the source creates the following data packet:
\begin{equation}
    \{ DT \concat \upsilon_{r1} \concat y'_0b_0 \}
\end{equation}
DT denotes the message type (data), $\upsilon_{r1}$ is the VCI number to identify next hop (note that only $r1$ knows
$\upsilon_{r1}$), and $y'_0 b_0$ is the initial message created by the source.
When $r1$ receives the message, based on its routing table,
it will send the following message to $r2$:
\begin{equation}
    \{ DT \concat \upsilon_{r2} \concat y'_0b_0 + y_1b_1 \}
\end{equation}
Then $r2$ will send the following message to $D$:
\begin{equation}
    \{ DT \concat \upsilon_{D} \concat y'_0b_0 + y_1b_1 + y_2b_2 \}
\end{equation}
Eventually, $D$ will recover the message $M = y'_0b_0 + y_1b_1 + y_2b_2 + y_3b_3$.
